NumS: Scalable Array Programming for the Cloud

Scientists increasingly rely on Python tools to perform scalable distributed memory array operations using rich, NumPy-like expressions. However, many of these tools rely on dynamic schedulers optimized for abstract task graphs, which often encounter memory and network bandwidth-related bottlenecks due to sub-optimal data and operator placement decisions. Tools built on the message passing interface (MPI), such as ScaLAPACK and SLATE, have better scaling properties, but these solutions require specialized knowledge to use. In this work, we present NumS, an array programming library which optimizes NumPy-like expressions on task-based distributed systems. This is achieved through a novel scheduler called Load Simulated Hierarchical Scheduling (LSHS). LSHS is a local search method which optimizes operator placement by minimizing maximum memory and network load on any given node within a distributed system. Coupled with a heuristic for load balanced data layouts, our approach is capable of attaining communication lower bounds on some common numerical operations, and our empirical study shows that LSHS enhances performance on Ray by decreasing network load by a factor of 2x, requiring 4x less memory, and reducing execution time by 10x on the logistic regression problem. On terabyte-scale data, NumS achieves competitive performance to SLATE on DGEMM, up to 20x speedup over Dask on a key operation for tensor factorization, and a 2x speedup on logistic regression compared to Dask ML and Spark's MLlib.

==> misc/preamble.tex <==
%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
% \setcopyright{acmcopyright}
% \copyrightyear{2021}
% \acmYear{2021}
% \acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
% \acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural
%   Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%   June 03--05, 2018, Woodstock, NY}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

==> misc/simplebnf.tex <==
%%
%% This is file `simplebnf.sty'.
%%
%% ---------------------------------------------------------------------------
%% The simplebnf package --- A simple package to format Backus-Naur form
%% Maintained by Jay Lee
%% E-mail: jaeho.lee@snu.ac.kr
%% Released under the MIT License.
%% ---------------------------------------------------------------------------
%%
\RequirePackage{expl3,xparse}
% mathtools is needed for the \Coloneqq simbol
\RequirePackage{mathtools}
\ProvidesExplPackage
  {simplebnf}
  {2019/12/23}
  {0.1.0}
  {A simple package to format Backus–Naur form}


\cs_generate_variant:Nn \seq_set_split:Nnn {NVn}

\tl_new:N \g__simplebnf_defeq_tl
\tl_gset:Nn \g__simplebnf_defeq_tl { \ensuremath{\Coloneqq} }

\tl_new:N \g__simplebnf_defor_tl
\tl_gset:Nn \g__simplebnf_defor_tl { \ensuremath{|} }

\seq_new:N \l__input_seq
\tl_new:N \l__term_tl
\tl_new:N \l__body_tl
\tl_new:N \l__keypairs_tl
\seq_new:N \l__keypairs_seq

\NewDocumentCommand \bnfexpr { m } { \texttt { #1 } }
\NewDocumentCommand \bnfannot { m } { \textit{ #1 } }

\NewDocumentEnvironment { bnfgrammar } { +b }
  {
    % Store the term to define grammar in \l__term_tl and the
    % (alternative form: annotion) keypairs in \l__keypairs_tl
    \regex_split:nnN { ::= } { #1 } \l__input_seq
    \seq_pop_left:NN \l__input_seq \l__term_tl
    \seq_pop_left:NN \l__input_seq \l__keypairs_tl

    % Store keypairs
    \seq_set_split:NnV \l__keypairs_seq { | } \l__keypairs_tl

    \begin{center}
      \tl_set:Nn \l__table_tl
        {
          \begin{tabular}{lcll}
            \bnfexpr { \l__term_tl } & \g__simplebnf_defeq_tl &
        }

      \bool_set_false:N \l_tmpa_bool

      \seq_map_inline:Nn \l__keypairs_seq
        {
          \bool_if:NTF \l_tmpa_bool
            { \tl_put_right:Nn \l__table_tl { \\ & \g__simplebnf_defor_tl & } }
            { \bool_set_true:N \l_tmpa_bool }

          \regex_split:nnNTF { : } { ##1 } \l_tmpa_seq
            {
              \seq_pop_left:NNT \l_tmpa_seq \l_tmpa_tl
                {
                  \tl_set:Nx \l_tmpa_tl { \bnfexpr { \l_tmpa_tl } }
                  \tl_put_right:NV \l__table_tl \l_tmpa_tl
                }

              \tl_put_right:Nn \l__table_tl { & }

              \seq_pop_left:NNT \l_tmpa_seq \l_tmpb_tl
                {
                  \tl_set:Nx \l_tmpb_tl { \bnfannot { \l_tmpb_tl } }
                  \tl_put_right:NV \l__table_tl \l_tmpb_tl
                }
            }
            {
              \tl_put_right:Nn \l__table_tl { \bnfexpr { ##1 } & }
            }
        }

      \tl_put_right:Nn \l__table_tl { \end{tabular} }
      \tl_use:N \l__table_tl
    \end{center}
  }
  { }

%% The MIT License (MIT)
%%
%% Copyright © 2019-2020 Jay Lee <jaeho.lee@snu.ac.kr>
%%
%% Permission is hereby granted, free of charge, to any person obtaining
%% a copy of this software and associated documentation files (the "Software"),
%% to deal in the Software without restriction, including without limitation
%% the rights to use, copy, modify, merge, publish, distribute, sublicense,
%% and/or sell copies of the Software, and to permit persons to whom the
%% Software is furnished to do so, subject to the following conditions:
%%
%% The above copyright notice and this permission notice shall be included
%% in all copies or substantial portions of the Software.
%%
%% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
%% EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES
%% OF MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
%% IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
%% DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
%% TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE
%% OR THE USE OR OTHER DEALINGS IN THE SOFTWARE.
%%
%% End of file `simplebnf.sty'.


==> src/063-motivation.tex <==
\section{Motivation}
\label{sec:motivation}

We observe that dynamic scheduling, such as those provided by Ray and Dask, are unable to take advantage of the structure of distributed memory numerical array and tensor algebra operations. Dynamic algorithms view array creation operations as collections of independent tasks, which frequently results in sub-optimal placement of data for elementwise and tensor algebra operations. In Dask, summation of several operands is performed by constructing a balanced tree, but this subgraph is constructed before data is mapped to worker processes, which can lead to data movement.

Several static algorithms exist~\cite{pblas, scalapack, slate} for a variety of basic linear algebra operations on distributed memory systems, which provide consistent and quantifiable performance properties over dynamic algorithms. 
% More than this: Key insight has to notes on hierarchical networks.
The key insight of this work is that the common theme among all static scheduling techniques for basic linear algebra operations is to maintain good load balancing, and minimize data movement. We’re motivated by this insight to design a general static scheduling algorithm for elementwise, reduction, linear and tensor algebra operations which explicitly optimizes for load balance and data movement. Our algorithm, named Load Simulated Hierarchical Scheduling (LSHS), greedily minimizes the maximum memory and network load over all worker processes by simulating the cost of operator placement decisions within a hierarchical network topology. Our algorithm is greedy because this optimization problem is NP-Complete by reduction from load balancing, which we show in section (A). In section (B), we provide a communication analysis of LSHS, Dask, and Ray for a collection of key numerical operations, showing that our algorithm has favorable theoretical properties. We support our theoretical analysis with an empirical ablation of LSHS, comparing our scheduling algorithm to Dask and Ray. We do this on the open source project NumS, a modular system which provides abstractions for implementing distributed numerical array operations on Dask and Ray both with and without their native schedulers. We describe in greater detail the NumS system in section (C). In the following section, we provide background knowledge on key distributed systems concepts, hierarchical network topologies, scheduling algorithms, fusion, n-dimensional arrays, and key concepts in distributed memory numerical array computing on MPI. 

\begin{figure}
    \centering
    \includegraphics[width=0.2\textwidth]{src/figures/placeholder.png}
    \caption{A computation graph depicting potential sub-optimal placement of the data and operations required to perform $\X^T \Y$, where both $\X$ and $\Y$ are partitioned row-wise into 4 blocks each. In a 2-node cluster consisting of 4 workers each, a dynamic scheduler is unable to provide any locality guarantees on initial or intermediate data placement. Purple vertices correspond to data/operations placed on node 1, and blue vertices correspond to data/operations placed on node 2.}
    \label{fig:inner-product-example}
\end{figure}

Figure \ref{fig:inner-product-example} illustrates a relatively simple example of what may occur when array operations are dynamically scheduled. A common operation which occurs when optimizing generalized linear models using Newton's method is $\X^T \Y$. Data is distributed to distinct workers for parallelism. When data and operator placement is delegated to a distributed system with dynamic scheduling, operands are often not co-located, resulting in greater memory and data movement requirements. Our example illustrates what happens in Dask for this operation (see Figure \ref{fig:ablation-performance} for empirical results). Every operation requires at least one inter-node object transfer, requiring $3\times$ more time than the theoretical lower bound we provide within our framework. This is also an example of the kind of operation for which SUMMA is sub-optimal: The computation will be carried out as a sequence of rank-1 updates to the output partition. With $4$ updates, and each update requiring 2 partitions, SUMMA requires $4$ object transmissions. On the other hand, SUMMA executes $\X \Y^T$ optimally. We provide a more detailed analysis of these algorithmic properties in Section \ref{sec:analysis}.

